Output Range Analysis for Deep Neural Networks

Deep neural networks (NN) are extensively used for machine learning tasks such as image classification, perception and control of autonomous systems. Increasingly, these deep NNs are also been deployed in high-assurance applications. Thus, there is a pressing need for developing techniques to verify neural networks to check whether certain user-expected properties are satisfied. In this paper, we study a specific verification problem of computing a guaranteed range for the output of a deep neural network given a set of inputs represented as a convex polyhedron. Range estimation is a key primitive for verifying deep NNs. We present an efficient range estimation algorithm that uses a combination of local search and linear programming problems to efficiently find the maximum and minimum values taken by the outputs of the NN over the given input set. In contrast to recently proposed "monolithic" optimization approaches, we use local gradient descent to repeatedly find and eliminate local minima of the function. The final global optimum is certified using a mixed integer programming instance. We implement our approach and compare it with Reluplex, a recently proposed solver for deep neural networks. We demonstrate the effectiveness of the proposed approach for verification of NNs used in automated control as well as those used in classification.

==> Methodology.tex <==
The technique developed here can be used to propagate a convex polyhedron through a  single output neural network with ReLU units as activation functions, in an exact sense. Consequently, for the multi-output  deep neural network this enables us to obtain tight convex over-approximations of the output range set with similar inputs. 
The technique that we use in order to propagate convex polyhedron through a single output can be divided into two phases. A gradient search over the input region, followed by a counter example guided hop, to get rid of any local optima that the gradient search might be stuck at. Henceforth we assume that the deep neural networks that we consider in this paper, have ReLU units as activation functions.

\subsection{Computing gradients for neural networks}

So, the idea is very simple. Let's say, we have  a neural network, $N$ described by the following tuple  $N = \{ L , D , W , B \}$. Where, $L$ represents the number of layers in the neural network, $D$ represents a set $\{ d_1, d_2, d_3,  \dots d_L \}$ represents the number of neurons we have at each of the layers in the neural network. $W$ represents the collection of weights in the neural network, indexed by , $\{ w^l_{jk} \}$, which basically represents the weight in the connection of the $k^{th}$ neuron in the $(l-1)^{th}$ layer to the $j^{th}$ neuron in the $l^{th}$ layer. And finally, $B$ denotes the set indexed as, $\{ b^l_j\}$, that is the bias of the $j^{th}$ neuron in the $l^{th}$ layer. Now, we assume that there is some activation function $\sigma$, which relates the weighted sum of the inputs to a neuron to the output of the particular neuron. That is the activation of the $j^{th}$ neuron in the $l^{th}$ layer, $a_j^l$ is related to the inputs of the neuron in the following way, 
\begin{equation}
\label{relu_equation}
a_j^l = \sigma ( \sum_{1 \leq k \leq d_{l-1} } w^l_{jk} a _k^{l-1} + b_j^l )
\end{equation}
Now, we know that for ReLU units describing the activation functions of the neural network, the $\sigma$ is given as the following function, $ \sigma(x) = max\{ 0, x \}$. 
\\
\begin{figure}
\begin{center}
\includegraphics[scale = 0.5]{Figures/simple_NN_1} 
\end{center}
\caption{A simple single input single output network}
\label{fig_init_example}
\end{figure} 

For ReLU units as activation functions, for any given neuron $j$ at the layer $l$, and the weights $w^l_{jk}$ , for $1 \leq k \leq d_{l-1}$, and a bias $b_j^l $ we can always, find a half space in terms of the activations (outputs) of the neurons in the preceding layer $(l-1)$. That is, each neuron only allows inputs to pass through, that satisfies a certain half space constraint in it's input region. Further it's output is simply the output of the same affine transformation it did in order to filter the inputs. 
Let us consider the neural network as given in Fig \ref{fig_init_example} example, further, we need to deduce the output range of the given network for an input in the range $(0, 15)$. In order to demonstrate this idea for the simple case, we observe that the single layer 2 neuron network defines the following linear inequalities in it's input space, : \{ $ x - 5 > 0 $ \}  and \{ $ - x + 5 > 0$ \}. That is it defines two distinct regions in the input space,\{ $ x \in (5, 15) $ \}  and \{ $ x \in (0, 5)$ \}. Hence, in a divide and conquer paradigm, we observe that the output range of the network, will be a union for the ranges for the two distinct cases. At first, let us restrict ourselves to the case when $x < 5$. For this case, we see that the network reduces to the one in Fig \ref{fig_init_example_reduced}. Hence, the output of the neural network for the inputs in the range from $(0, 5)$ simply reduces to $ y = x - 5.0$. Thus, the output range in this is case is $(0,5)$. Similarly for the case in which $x > 5.0$ we see that the output $y = x - 5 $. Hence, in this case the range reduces to $(0,10)$. Thus, the overall range of the network reduces to $(0, 10)$. There are two interesting observation that can be made from the above deduction for this particular example: One, identifying what the half space is that keeps, a certain neuron in an "ON" state, and the other in an "OFF" can help us get rid of both the neurons in the first (and only) layer, and two, depending on what the transformation was done by the "ON" neuron, can help us determine, what the weight and biases should be when we connect the input neuron, directly to the output neuron. Once, we have have determined that, the output of the neural network becomes a simple linear combination of the inputs, and deducing the range is just a linear programming problem then. 
\begin{figure}
\begin{center}
\includegraphics[scale = 0.5]{Figures/simple_NN_1a} 
\end{center}
\caption{For the case $x < 5.0$}
\label{fig_init_example_reduced}
\end{figure} 

Moving forward, if we have a multi layer neural network, we can easily identify the number of regions in the input space that first layer of the CNN, subdivides into. These regions are identified as a set of linear inequalities defining a convex polyhedron. Once, we have done this, and identified all these possible sub-regions, for each of the sub-regions we identify what the weights and biases should be that goes on to the neurons in the second layer, if we were to keep the CNN's output undisturbed in some particular region, without the involvement of the first layer. 

Let us demontrate this idea with an example. For the CNN, as shown in Fig \ref{fig_multi_layer_example}, we see that it has 2 inputs, and multiple layers, and the first layer has only two neurons, with the weights and biases as shown. Now, let us assume we need to find out the range of the output neuron for an input region in the box $[0,1]^2$. Since, there are 2 neurons in the first layer we observe that the input region can be split into at most $2^2$ subregions, all of which fall into the input polyhedron that we want to propagate. The 4 regions are labeled in Fig \ref{fig_multi_layer_example_input_space}, and can be defined by the following inequalities, (SR: Sub Region) SR-1: $ (x + y -1.0 < 0.0) \wedge ( x - y < 0.0 )$, SR-2: $ (x + y -1.0 > 0.0) \wedge ( x - y < 0.0 )$, SR-3: $ (x + y -1.0 > 0.0) \wedge ( x - y > 0.0 )$ and SR-4: $ (x + y -1.0 < 0.0) \wedge ( x - y > 0.0 )$.    
\\

Now, if we want to get rid of layer 1, of the network, and figure out what the network should like if we restrict ourselves to just one of the subregions, we can do so by carrying forward the effect of the "ON" neurons, in layer 1, and computing the weights and biases. For example if we want to figure out what the weights and biases should be if we want to connect the inputs directly to the first neuron in the 2nd layer, while we are in SR-3, we can do the following: since, in SR-3 both the neurons in the input layer are active we simply compute the output of both the neurons in a symbolic sense and take a weighted sum of them according to the weights connecting them to the 1st neuron in the 2nd layer. Thus, we have the following, let $O_1$ and $O_2$ be the output of the neurons in the 1st layer. Hence, the output $z$ as given in Fig \ref{fig_multi_layer_example}, will be $0.2 \times O_1 + 0.3 \times O_2 + 0.0$. Now, $O_1 = x - y$ and $O_2 = x + y - 1$. Thus, we get $z = 0.5 \times x + 0.1 \times y - 0.3$. The network after removing the first layer has been shown in Fig \ref{fig_multi_layer_example_layer_2}. We just show the effect on one of the neurons in layer 2 to keep the example simple.
\begin{figure}[h]
\begin{center}
\includegraphics[scale = 0.5]{Figures/simple_NN_2} 
\end{center}
\caption{A multilayer CNN }
\label{fig_multi_layer_example}
\end{figure} 
\begin{figure}[h]
\begin{center}
\includegraphics[scale = 0.5]{Figures/simple_NN_2a} 
\end{center}
\caption{Input region splitting for the first layer}
\label{fig_multi_layer_example_input_space}
\end{figure} 
\begin{figure}[h]
\begin{center}
\includegraphics[scale = 0.5]{Figures/simple_NN_2b} 
\end{center}
\caption{Reduced after removing layer 1 for input subregion: 3}
\label{fig_multi_layer_example_layer_2}
\end{figure} 
Thus, for each sub region, we will have a copy of the CNN which would represent, what the CNN would look like without the first layer. Now, once we have done that with the first layer we can continue doing this for the second layer, which becomes the new first layer , until we have exhausted all of the layer, and then take a max over all the sub region we have identified. But, doing so has a huge drawback. For each layer the number of subregions we identify is in the worst case, exponential in the number of neurons in the layer, and this happens for each subregion we identify and thus, even for a moderately sized network, the number of subregions is exponential in the total number of neurons. 
But, there is something we realize from the above discussion, the CNN with ReLU activation functions, essentially divides the input space into a potentially large number of subregions, and the output of the network is just a simple linear transformation on that subregion. Hence, for a point  in the input space, if we compute the network output , we can easily figure out for each layer which of the neurons are "ON" and which ones are "OFF". Based, on that information, if we can get rid of each layer starting with the first (left most layer), and we can identify this subregion, exactly. Once, that is done we can compute the minima and maxima for this subregion, since now the output will be a linear combination of the inputs and figuring out the minima and maxima, reduces to an Linear Program. Another useful information that we can derive from this is the actual gradient of the  network output, in terms of the inputs. This gradient, along with the maxima and minima are probably the most valuable piece of information we have about the behavior of the network locally, the boundaries of which are formally known. 
\\
Thus, given an input space , we can easily randomly sample a point in the input space and compute the local gradient and use that to guide us to an extrema. But, as is well known, this method has a serious pitfall of being stuck at a local optima. To get out of such a local optima that we might be stuck at, all we try to hop out of such a point using a counter example. The details of which has been explained in the next subsection.

\subsection{Counter example guided Hopping}

A recent result on falsifying CNN's  was, \cite{Reluplex}, which uses SMT techniques to exhaustively search for a satisfying assignment from the input set to the output set. That is, if the input sets and output sets are given as interval valued sets, it can return a satisfying assignment if any. The method is complete in the sense that if there are no satisfying assignment the method should come back with an UNSAT. But, in this paper we adopt another route , mentioned in \cite{MILP_encoding} which gives added flexibility in using convex polyhedra as input sets. This method has some other advantages which will be apparent later on. 
\begin{figure}[h]
\begin{center}
\includegraphics[scale = 0.35]{Figures/Counter_Example_guided_hop} 
\end{center}
\caption{Counter Example Guided Hop}
\label{fig_counter_example_guided_hop}
\end{figure} 
The MILP encoding of the NN to generate satisfying assignments, from an input convex polyhedra to an output convex polyhedra is as follows: Let $z$ be the number of layers in a CNN, and $i$ in the range, $0 \leq i \leq z$. Now, for $x^{i-1}$ and $x^{i}$ be the outputs of the CNN for layer $(i-1)$ and $i$, and $\delta^{i}$ a vector of binary variables, the encoding for a layer $i$ is defined as the following, 

\begin{equation}
\label{MILP_formulation}
\begin{aligned}
C_i = \{ & x_j^{i} \geq W_j^i x^{i-1} + b_j^i, \\
		 & x_j^{i} \leq W_j^i x^{i-1} + b_j^i + M\delta_j^i, \\
         & x_j^i \geq 0, \\
         & x_j^i \leq M(1 - \delta_j^i) \text{		}| j = 1\dots |L^i|
\}
\end{aligned}
\end{equation}
Where $M$ is a sufficiently large constant. Depending on the size of the inputs polyhedron, an upper bound for $M$ can be easily deduced. In practice, it can be also be chosen as a large a enough constant. Thus, the MILP encoding of the network is nothing but, a union of the individual constraints for each layer, for all the layers of the network. That is the network encoding $N_e = \cup_{i=1}^k C_i$. 
Thus, for some polyhedral input space, being encoded by the constraint $C_{in}$, and an output range for the polyhedra encoded as $C_{out}$, the MILP feasibility question can be posed as a feasibility of the constraint $C = C_{in} \cup N_e \cup C_{out}$. 

As was shown in \cite{Reluplex}, the problem of finding satisfying assignments from an input interval to an output interval, which respects the network constraints, was NP complete. The MILP encoding of the above problem does not make it any more simpler, since, as is well known mixed integer linear programming is NP complete.

Thus each time the gradient search leads us to some optima (say $M^*$), at a point $x^*$, we encode the output constraint as, ( assuming $y$ is the output of the network), $y > M^*$ , if we are looking for the maxima, and $y < M^*$, if we are looking for the minima. Hence, as was shown in Fig \ref{fig_counter_example_guided_hop}, the MILP solver comes back with a satisfying assignment where we resume our gradient search from. Thus, we continue in this process until the MILP solver comes back and says that the constraints are infeasible. At which point we stop and declare that we have found the optima. 

Now, in practice we know that MILP solver perform a combinatorial search over the integer constraints, to find a feasible solution to the constraints. Thus, more the number of calls we make to the MILP solver, slower the algorithm gets. Also, if we indeed reach the real optima while doing the gradient search, the algorithm shall terminate with just a single call to the MILP solver. Thus, if we can perform multiple gradient searches in parallel, and take the most optimum solution, then there is high probability that we indeed reach the real optima. 

Further, another interesting observation can be made about the network encoding $N_e$. If we do an LP relaxation of network encoding, and the LP problem is infeasible then we can be rest assured that the MILP is infeasible. This is important since all we need is a certificate of in-feasibility at the end in order to prove that we have indeed reached the real optima. This makes the task of obtaining a certificate of infeasibility P time, since LP is P time. 
\begin{figure}[h]
\begin{center}
\includegraphics[scale = 0.35]{Figures/main_algorithm} 
\end{center}
\caption{Algorithm}
\label{fig_algorithm}
\end{figure} 





